Stability Does Not Mirror Plasticity: A Module-Level View of Declarative and Procedural Learning in Transformers

Plasticity and stability in continual learning are typically studied at the entire-model level and in a task-agnostic manner, yet prior work has reported divergent conclusions across settings. Inspired by cognitive distinctions between declarative and procedural memory, we instead study how plasticity and stability vary across transformer modules and task types. In a controlled synthetic environment with clean measurement, we show a double dissociation: query-key (QK) and value-output (VO) projections are the most plastic on procedural tasks, whereas MLPs are the most plastic on declarative memorization. Stability, however, does not simply mirror plasticity: when learning a new procedure, updating QK retains over half of the stored declarative memory, while updating MLPs retains far less and updating VO loses roughly four-fifths. Targeted module reset-and-recovery experiments explain this asymmetry: plasticity tracks which module is best suited to a task's primary computation or storage, whereas stability depends on all ways the existing capability relies on that module, including access to information stored in other modules. Experiments on a realistic model and tasks broadly echo these asymmetric dynamics. Overall, our work shows that plasticity and stability depend on different aspects of a module's functional role, offering a task-dependent, module-level perspective on continual learning.

==> sec/plot_tex/realistic_1.tex <==
% Preamble (once):  \usepackage{graphicx}  \usepackage{subcaption}
% One row: the three procedural learning curves (plasticity) and the knowledge-injection scatter (declarative trade-off).
% All four files are 2.75 x 2.2 in, so equal widths print them at one scale.
\begin{figure}[t]
  \centering
  \begin{subfigure}[t]{0.24\linewidth}
    \centering
    \includegraphics[width=\linewidth]{figs/crux_learning_curve.pdf}
    \caption{Code Cxecution}
    \label{fig:crux_learning_curve}
  \end{subfigure}\hfill
  \begin{subfigure}[t]{0.24\linewidth}
    \centering
    \includegraphics[width=\linewidth]{figs/sgd_learning_curve.pdf}
    \caption{Dialogue Conversion}
    \label{fig:sgd_learning_curve}
  \end{subfigure}\hfill
  \begin{subfigure}[t]{0.24\linewidth}
    \centering
    \includegraphics[width=\linewidth]{figs/ctx_learning_curve.pdf}
    \caption{Context Following}
    \label{fig:ctx_learning_curve}
  \end{subfigure}\hfill
  \begin{subfigure}[t]{0.24\linewidth}
    \centering
    \includegraphics[width=\linewidth]{figs/qa_learning_curve.pdf}
    \caption{Knowledge Injection}
    \label{fig:qa_learning_curve}
  \end{subfigure}
  \caption{Realistic setting (Qwen2.5-0.5B, no replay). (a--c) Task score while learning each procedural task with one module updated. (d) Facts learned vs.\ SGD skill retained after injecting facts into the SGD model.}
  \label{fig:realistic}
\end{figure}


==> sec/plot_tex/realistic_2.tex <==
\begin{figure}[t]
  \centering
  \begin{subfigure}[t]{0.32\linewidth}
    \centering
    \includegraphics[width=\linewidth]{figs/real_stab_crux.pdf}
    \caption{After CRUXEval-O.}
    \label{fig:real-stab-crux}
  \end{subfigure}\hfill
  \begin{subfigure}[t]{0.32\linewidth}
    \centering
    \includegraphics[width=\linewidth]{figs/real_stab_sgd.pdf}
    \caption{After SGD.}
    \label{fig:real-stab-sgd}
  \end{subfigure}\hfill
  \begin{subfigure}[t]{0.32\linewidth}
    \centering
    \includegraphics[width=\linewidth]{figs/real_stab_kc.pdf}
    \caption{After Knowledge Conflict.}
    \label{fig:real-stab-kc}
  \end{subfigure}
  \caption{Knowledge retained (four benchmarks) after learning each procedural task with one module updated; background bands mark the updated module.}
  \label{fig:real-stab}
\end{figure}


==> sec/plot_tex/recovery_bfs.tex <==
\begin{wrapfigure}{r}{0.66\textwidth}
    \centering
    \begin{subfigure}[t]{0.48\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figs/recovery_bfs.pdf}
        \caption{Recovery Process of BFS}
        \label{fig:reset_bfs}
    \end{subfigure}\hfill
    \begin{subfigure}[t]{0.48\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figs/recovery_bfs_control.pdf}
        \caption{Control Group}
        \label{fig:recovery_bfs_control}
    \end{subfigure}
    \caption{Module-wise reset-and-recovery of procedural skill.}
    \label{fig:recovery_bfs_wrap}
\end{wrapfigure}


==> sec/plot_tex/recovery_mem.tex <==
\begin{wrapfigure}{r}{0.66\textwidth}
    \centering
    \begin{subfigure}[t]{0.48\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figs/recovery_mem_full_load.pdf}
        \caption{Recovery process}
        \label{fig:recovery_mem_full_load}
    \end{subfigure}\hfill
    \begin{subfigure}[t]{0.48\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figs/recovery_mem.pdf}
        \caption{Recovery across loads}
        \label{fig:recovery_mem}
    \end{subfigure}
    \caption{Module-wise reset-and-recovery of declarative memory.}
    \label{fig:recovery_memory_wrap}
\end{wrapfigure}


==> sec/plot_tex/synthetic_1.tex <==
% preamble: \usepackage{graphicx} \usepackage{subcaption}
\begin{figure}[t]
  \centering
  \begin{subfigure}[t]{0.67\linewidth}
    \centering
    \includegraphics[width=\linewidth]{figs/syn_panel_plast_proc.pdf}
    \caption{Procedural plasticity: DFS exact match during Stage-2 training.}
    \label{fig:syn-plast-proc}
  \end{subfigure}\hfill
  \begin{subfigure}[t]{0.33\linewidth}
    \centering
    \includegraphics[width=\linewidth]{figs/syn_panel_stab_proc.pdf}
    \caption{Procedural stability: old memory retained after learning DFS.}
    \label{fig:syn-stab-proc}
  \end{subfigure}

  \vspace{0.5em}

  \begin{subfigure}[t]{0.67\linewidth}
    \centering
    \includegraphics[width=\linewidth]{figs/syn_panel_plast_decl.pdf}
    \caption{Declarative plasticity: new memory stored per trainable parameter.}
    \label{fig:syn-plast-decl}
  \end{subfigure}\hfill
  \begin{subfigure}[t]{0.33\linewidth}
    \centering
    \includegraphics[width=\linewidth]{figs/syn_panel_stab_decl.pdf}
    \caption{Declarative stability: old BFS accuracy after learning new memory.}
    \label{fig:syn-stab-decl}
  \end{subfigure}
  \caption{Plasticity (left) and stability (right) by updated module in the synthetic testbed,
    for the procedural (top) and declarative (bottom) directions. Mean of three seeds; no replay.}
  \label{fig:synthetic}
\end{figure}

==> sec/plot_tex/synthetic_2.tex <==
\begin{figure}[t]
  \centering
  \begin{subfigure}[t]{0.24\linewidth}
    \centering
    \includegraphics[width=\linewidth]{figs/syn_reset_mem_qk75.pdf}
    \caption{75\% of QK}
    \label{fig:reset-mem-qk75}
  \end{subfigure}\hfill
  \begin{subfigure}[t]{0.24\linewidth}
    \centering
    \includegraphics[width=\linewidth]{figs/syn_reset_mem_mlp75.pdf}
    \caption{75\% of MLP}
    \label{fig:reset-mem-mlp75}
  \end{subfigure}\hfill
  \begin{subfigure}[t]{0.24\linewidth}
    \centering
    \includegraphics[width=\linewidth]{figs/syn_reset_mem_mlpqk.pdf}
    \caption{100\% of MLP+QK}
    \label{fig:reset-mem-mlpqk}
  \end{subfigure}\hfill
  \begin{subfigure}[t]{0.24\linewidth}
    \centering
    \includegraphics[width=\linewidth]{figs/syn_reset_mem_full1p5.pdf}
    \caption{1.5$\times$ full-model}
    \label{fig:reset-mem-full1p5}
  \end{subfigure}
  \caption{Held-out memory recovered after resetting one module (legend) and retraining the full model on a 10\% replay support (first 3{,}000 optimizer steps; step 0 = right after the reset). Seed 44.}
  \label{fig:reset-mem}
\end{figure}


==> sec/plot_tex/synthetic_3.tex <==
\begin{figure}[t]
  \centering
  \begin{subfigure}[t]{0.48\linewidth}
    \centering
    \includegraphics[width=\linewidth]{figs/syn_reset_bfs_trained.pdf}
    \caption{From the trained model (BFS + memory).}
    \label{fig:reset-bfs-trained}
  \end{subfigure}\hfill
  \begin{subfigure}[t]{0.48\linewidth}
    \centering
    \includegraphics[width=\linewidth]{figs/syn_reset_bfs_memonly.pdf}
    \caption{Control: from the memory-only checkpoint.}
    \label{fig:reset-bfs-memonly}
  \end{subfigure}
  \caption{Held-out BFS token accuracy while retraining the full model on BFS after resetting one module (legend); the dashed red line marks step 96.}
  \label{fig:reset-bfs}
\end{figure}

